Computation-Aware Data Aggregation

Data aggregation is a fundamental primitive in distributed computing wherein a network computes a function of every nodes' input. However, while compute time is non-negligible in modern systems, standard models of distributed computing do not take compute time into account. Rather, most distributed models of computation only explicitly consider communication time. In this paper, we introduce a model of distributed computation that considers \emph{both} computation and communication so as to give a theoretical treatment of data aggregation. We study both the structure of and how to compute the fastest data aggregation schedule in this model. As our first result, we give a polynomial-time algorithm that computes the optimal schedule when the input network is a complete graph. Moreover, since one may want to aggregate data over a pre-existing network, we also study data aggregation scheduling on arbitrary graphs. We demonstrate that this problem on arbitrary graphs is hard to approximate within a multiplicative $1.5$ factor. Finally, we give an $O(\log n \cdot \log \frac{\mathrm{OPT}}{t_m})$-approximation algorithm for this problem on arbitrary graphs, where $n$ is the number of nodes and $\mathrm{OPT}$ is the length of the optimal schedule.

==> abstract.tex <==
\title{A Computational Approach to Organizational Structure}


\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\author[ ]{Bernhard Haeupler\thanks{Supported in part by NSF grants CCF-1527110, CCF-1618280 and NSF CAREER award CCF-1750808.}, D. Ellis Hershkowitz\samethanks, Anson Kahng\thanks{Supported in part by NSF grants IIS-1350598, IIS-1714140, CCF-1525932, and CCF-1733556; by ONR grants N00014-16-1-3075 and N00014-17-1-2428; and by a Sloan Research Fellowship and a Guggenheim Fellowship.}, Ariel D. Procaccia\samethanks\\ 
Computer Science Department\\
Carnegie Mellon University\\
\texttt{\{haeupler,dhershko,akahng,arielpro\}@cs.cmu.edu}}
\date{}
\maketitle
\begin{abstract}
	An organizational structure determines how an organization arranges and manages its individuals. %Because individuals in an organization take time to both perform tasks and communicate, organizational structure must take both computation and communication into account. 
	Sociologists have studied organizational structure from an empirical perspective for decades, but their work has been limited by small sample sizes. By contrast, we study organizational structure from a computational and theoretical perspective. 
	
	Specifically, we introduce a model of organizations that involves both computation and communication, and captures the spirit of past sociology experiments. %This model allows us to reason about the optimal organizational structure and workflow for any number of people. 
	In our model, each node in a graph starts with a \wad, and at any time can either perform computation to merge two \wads in $t_c$ time, or perform communication by sending a \wad to a neighbor in $t_m$ time. We study how to schedule computation and communication so as to merge all \wads as quickly as possible. 
	
	As our first result, we give a polynomial-time algorithm that optimally solves this problem on a complete graph. This result characterizes the optimal graph structure---the edges used for communication in the optimal schedule---and therefore informs the optimal design of large-scale organizations. Moreover, since pre-existing organizations may want to optimize their workflow, we also study this problem on arbitrary graphs. We demonstrate that our problem on arbitrary graphs is not only NP-complete but also hard to approximate within a multiplicative $1.5$ factor. Finally, we give an $O(\log n \cdot \log \frac{\OPT}{t_m})$-approximation algorithm for our problem on arbitrary graphs, where $n$ is the number of nodes and $\OPT$ is the length of the optimal schedule.
	%Organizations with many members must coordinate both who performs tasks and how members communicate. %For example, a company must coordinate not only which employees communicate but also which employees perform which tasks. 
	%Similarly, a network of many computers must coordinate not only which computers perform computation, but also when and how computers communicate. 
	%
	%We study how to optimally coordinate computation and communication in an organization or network. In particular, we introduce the \gum model, which represents members of a network or organization as nodes in a graph where edges dictate which nodes can communicate.
	%In our model, \emph{both} the computation performed by nodes and the communication between nodes take time. We study the problem of producing a minimal-time \gum schedule that dictates when nodes should compute and when and with whom they should communicate so as to complete a task. We show that this problem can be optimally solved in polynomial time on complete graphs. However, on general graphs, we demonstrate that not only is the problem NP-hard, but also that no polynomial-time algorithm can produce a schedule using less than $1.5$ times as much time as the optimal schedule unless $\text{NP} \in \text{DTIME}\left(n^{O(\log \log n)} \right)$. Finally, we present a polynomial-time algorithm that produces a schedule using $O\left(\log n \cdot \log \tfrac{\OPT}{t_m} \right)$ multiplicatively more time than the optimal schedule for any input graph where $t_m$ is the time communication takes and $\OPT$ is the time taken by the optimal schedule.
\end{abstract}


% We build on previous work in the field of distributed computation, with one novel difference. Most models of distributed computation assume that nodes have access to unbounded computation. In doing so, these models distill out exactly how much communication is necessary to accomplish certain tasks in a distributed manner. However, myopically focusing on communication fails to capture a difficulty of real-world distributed computation: how communication and computation interact. In this work, we introduce a model of distributed computation in which nodes have limited computation, as well as a problem that encapsulates the crux of organizational problem-solving, the \gum problem. We then optimally solve \gum on complete graphs, demonstrate NP-hardness and hardness of approximation of \gum on arbitrary graphs, and finally present an approximation algorithm for solving \gum on arbitrary graphs.


